Survey of Disaggregated Memory: Cross-layer Technique Insights for Next-Generation Datacenters

The growing scale of data requires efficient memory subsystems with large memory capacity and high memory performance. Disaggregated architecture has become a promising solution for today's cloud and edge computing for its scalability and elasticity. As a critical part of disaggregation, disaggregated memory faces many design challenges in many dimensions, including hardware scalability, architecture structure, software system design, application programmability, resource allocation, power management, etc. These challenges inspire a number of novel solutions at different system levels to improve system efficiency. In this paper, we provide a comprehensive review of disaggregated memory, including the methodology and technologies of disaggregated memory system foundation, optimization, and management. We study the technical essentials of disaggregated memory systems and analyze them from the hardware, architecture, system, and application levels. Then, we compare the design details of typical cross-layer designs on disaggregated memory. Finally, we discuss the challenges and opportunities of future disaggregated memory works that serve better for next-generation elastic and efficient datacenters.

==> Contents/Heterogeneity.tex <==
\section{Heterogeneous Far Memory} \label{sec-heterogeneous}
With the development of computing accelerators and memory chips, the construction and research of heterogeneous far-memory environments become very important. 

%On the one hand, new acceleration devices have higher performance than CPUs, but more limited memory space. Accelerators urgently need high-performance memory scaling techniques. On the other hand, the development of new memory technologies increases the available data access paths, which requires fine-grained hybrid memory management to support both high-performance computation and efficient memory usage.


\subsection{GPU Far Memory Management} 
GPUs require orders-of-magnitude higher memory bandwidth than traditional CPU-based systems \cite{2022ai-hpca}. However, the memory space of GPU is still limited and the capacity of such high-bandwidth memory tends to be relatively small. There are several GPU far memory access paths, including CPU memory, NVLink-based remote GPU memory, direct-storage-based storage space, direct-rdma-based remote memory, etc.

\subsubsection{Page swap on unified memory}


In GPU far memory architecture, Unified Virtual Memory (UVM) is an essential way to integrate GPU and CPU memory spaces. This arrangement facilitates data sharing between CPU and GPU, with no transfer exposed to apps and users. Recent work focuses on leveraging CPU memory for specific purposes and optimizing current management strategies.

Swap Advisor \cite{swapadvisor} proposes a general swapping mechanism that can swap deeper and wider neural networks on limited GPU memory. The memory consumption is reduced by smartly swapping the model parameters that are updated at the end of each iteration and used by the next iteration. To optimize GPU's memory access overhead, Grus \cite{wang-grus} co-utilizes different memory-sharing operations of CUDA UVM when running graph workloads. Shao et al.  \cite{shao-icpe} investigated the implications of GPU UVM oversubscription. They evaluate the performance sensitivity of applications with over-subscribed memory size on GPU. Some works adopt memory efficient techniques with static and dynamic scheduling strategies to execute large-scale graph random walk on GPU and CPU memory\cite{wang-skywalker,flowwalker-mei}.  Soroush et al  \cite{co-optimizing} explored the hidden performance implication of GPU memory management methods and developed a performance model that can predict system overhead for each memory management method.  



% It can also carefully handle the intermediate results including activation, gradient, and error tensors for smart data swap.

% Swap Advisor \cite{swapadvisor} proposes a general swapping mechanism in which any tensor can be swapped in/out under memory pressure which helps to swap the deeper and wider neural networks with better accuracy but limited GPU memory. They model the deep learning computation as a dataflow graph, which performs joint optimization along 3 dimensions based on the given dataflow graph: operator scheduling, memory allocation, and swap decisions.  They reduce the DNN’s memory consumption by 1) smartly swapping the model parameters that are updated at the end of an iteration and used by the next iteration; 2) carefully handling the intermediate results  including activation, gradient and error tensors, of which the latter two are only present in training but not in inference; and 3) managing the scratch space which is up to one gigabyte as a small fraction of total memory use.

% Grus \cite{wang-grus} analyzes the impact of several unified virtual memory (UVM) interfaces on graph workloads and proposes optimized adjustments for better performance. Shao et al.  \cite{scm-uvm} we attempt to analyze and explain the implications of GPU UVM oversubscription. They evaluate the performance sensitivity of applications with over-scribed memory size on GPU, and they find that co-running applications make memory competition worse in this case.  

% Soroush et al  \cite{co-optimizing} sets out to explore the hidden performance implication of GPU memory management methods of integrated CPU/GPU architecture. Through a series of experiments on micro-benchmarks and real-world workloads, they analyze application characteristics and develop a performance model that can predict system overhead for each memory management method.  They also propose a runtime scheduler that can significantly relieve the system memory pressure and reduce the multitasking co-run response time by conducting per-task memory management policy switching and kernel overlapping.


\subsubsection{GPU direct memory access}
The integration of GPU memory with high-speed storage devices like SSDs and NVMe drives is another frontier in GPU far memory management. Besides storage devices with sufficient bandwidth for memory management, novel network technology and hardware like RDMA allow data access faster and lower-costly. Current work focuses on reducing data transfer volume by achieving higher offload and prefetch efficiency and achieving higher bandwidth and lower latency with hardware and software methods.

GPU Direct-storage (GDS) techniques \cite{direct-storage} create a direct data path between local or remote storage, such as NVMe or NVMe over Fabrics (NVMe-oF), and GPU memory. By enabling direct-memory access (DMA) near the network adapter or storage, it moves data into or out of GPU memory—without burdening the CPU. 
GPUDirect RDMA  \cite{direct-rdma} is a technology introduced in Kepler-class GPUs and CUDA 5.0 that enables a direct path for data exchange between the GPU and a third-party peer device using standard features of PCI Express.  BAM  \cite{bam} proposes a big accelerator memory system that enables GPUs to orchestrate high-throughput, fine-grain SSD storage access. It mitigates I/O traffic amplification by enabling the GPU threads to read or write small amounts of data on-demand through highly concurrent I/O queues. 

%Examples of third-party devices are: network interfaces, video acquisition devices, storage adapters.
% BAM  \cite{bam} proposes big accelerator memory system that enables GPUs to orchestrate high-throughput, fine-grain accesses into NVMe Solid State Drives (SSDs) in a new system architecture. (1)  BaM infrastructure software running on GPUs can identify and communicate the fine-grain accesses at a sufficiently high rate to fully utilize the underlying storage devices, (2) even with consumer-grade SSDs, a BaM system can support application performance that is competitive against a much more expensive DRAM-only solution, and (3) the reduction in I/O amplification can yield significant performance benefit. These results are achieved by introducing high-throughput GPU data structures like queues and software caches that exploit the massive thread-level parallelism in GPUs to hide long latencies to the SSDs.

% GPU Direct-storage techniques \cite{direct-storage} creates a direct data path between local or remote storage, such as NVMe or NVMe over Fabrics (NVMe-oF), and GPU memory. By enabling a direct-memory access (DMA) engine near the network adapter or storage, it moves data into or out of GPU memory—without burdening the CPU.

% GPUDirect RDMA  \cite{direct-rdma} is a technology introduced in Kepler-class GPUs and CUDA 5.0 that enables a direct path for data exchange between the GPU and a third-party peer device using standard features of PCI Express. Examples of third-party devices are: network interfaces, video acquisition devices, storage adapters.

% ZeRO-Infinity  \cite{Zero-infinity} is a novel heterogeneous system technology that leverages GPU, CPU, and NVMe memory to allow for unprecedented model scale on limited resources without requiring model code refactoring.



\subsubsection{Heterogeneous memory pool for GPU}

Buddy Compression \cite{buddycompression}  leverages compression to utilize a larger buddy memory from the host or DM, effectively increasing the memory capacity of the GPU. It compresses the offloaded memory as compressed memory locally and utilizes buddy storage with alternatives, including CPU memory, DM, unused peer GPU memory, and NVMe SSDs. ZeRO-Infinity  \cite{Zero-infinity} is a novel heterogeneous system technology that leverages GPU, CPU, and NVMe memory to allow for unprecedented model scale on limited resources without requiring model code refactoring.


\subsubsection{Shared memory pool for multi-GPU}


Multi-GPU configurations amplify the computational power of many GPUs for serving large-scale applications like Large Language Model (LLM). However, they introduce challenges in managing memory throughout GPUs and accelerate computation and communication. Recent work aims to use a multi-GPU system for distributed deep learning and optimize memory management and communication mechanisms.
COARSE  \cite{coarse-hpca22} is a disaggregated memory extension for distributed deep learning (DL) training on multi-GPU. It proposes dynamic tensor routing and partitioning to fully utilize the non-uniform serial bus bandwidth varied across different cloud computing systems. %It designs a deadlock avoidance and dual synchronization to ensure high-performance parameter synchronization. 
MC-DLA  \cite{micro2018beyond} proposes a memory-centric deep learning system architecture that aggregates a pool of capacity-optimized memory modules within the device-side interconnect for transparent memory capacity expansion. %This architecture allows the accelerators to access the memory nodes via the high-bandwidth links, thus the performance overhead of virtualizing memory can be substantially reduced.
Griffin  \cite{griffin} is a holistic hardware-software solution to improve the performance of NUMA multi-GPU systems. Griffin introduces programmer transparent modifications to both the IOMMU and GPU architecture, supporting efficient runtime page migration. 

%LaySA \cite{zhao2021bridging} proposes a layer-centric memory-efficient distributed sparse communication mechanism and addresses the contradiction between memory management and sparse communication optimization.% This scheme can fill the gap in relation to multiple resource optimization in distributed GPU-based training systems. 



% \textit{Problems}: bandwidth, load balance, page migration frequency

% COARSE  \cite{coarse-hpca22} is a disaggregated memory extension for distributed deep learning (DL) training on multi-GPU. It proposes dynamic tensor routing and partitioning to fully utilize the non-uniform serial bus bandwidth varied across different cloud computing systems. It designs a deadlock avoidance and dual synchronization to ensure high-performance parameter synchronization. 

%  MC-DLA  \cite{micro2018beyond} proposes a memory-centric deep learning system architecture that aggregates a pool of capacity-optimized memory modules within the device-side interconnect for transparent memory capacity expansion. This architecture allows the accelerators to access the memory nodes via the high-bandwidth links, thus the performance overhead of virtualizing memory can be substantially reduced. At the same time, MC-DLA connects the accelerators and the memory nodes in a manner that maximizes inter-device communication bandwidth so that DC-DLA’s high efficiency in conducting collective communication operations is maintained. 

%  Griffin  \cite{griffin} states that current multi-GPU systems rely on a first-touch Demand Paging scheme, where memory pages are migrated from the CPU to the GPU on the first GPU access to a page. this mechanism suffers from two major drawbacks: 1) imbalance in the page distribution across multiple GPUs, and 2) inability to move the page to the GPU that uses it most frequently. Both of these problems lead to load imbalance across GPUs, degrading the performance of the multi-GPU system. Griffin  \cite{griffin} is a holistic hardware-software solution to improve the performance of NUMA multi-GPU systems. Griffin introduces programmer transparent modifications to both the IOMMU and GPU architecture, supporting efficient runtime page migration based on locality information. In particular, Griffin employs a novel mechanism to detect and move pages at runtime between GPUs, increasing the frequency of resolving accesses locally. To ensure better load balancing across GPUs, Griffin employs a Delayed First Touch Migration policy that ensures pages are evenly distributed across multiple GPUs. 

% LaySA \cite{zhao2021bridging} proposes a layer-centric memory-efficient distributed sparse communication mechanism in terms of both system memory and bandwidth resources.  Firstly, to tackle the memory ballooning issue caused by sparse communication, the existing memory reuse strategy is refined, and the data object of the memory optimization is augmented and redefined. Secondly, a mirror weight update mechanism is proposed to address the contradiction between memory management and sparse communication optimization for weight gradients. Our scheme, which involves the deep integration and collaborative execution of these two types of strategies, can fill the gap in relation to multiple resource optimization in distributed GPU-based training systems. 

% \subsubsection{GPU + CPU(UVM)}
% In the context of GPU far memory architecture, Unified Virtual Memory (UVM) is an essential way to integrate GPU and CPU memory spaces. This arrangement facilitates data sharing between CPU and GPU, with no transfer exposed to apps and users. Recent work focuses on leveraging CPU memory for specific purposes and optimizing current management strategies.

% Swap Advisor \cite{swapadvisor} proposes a general swapping mechanism in which any tensor can be swapped in/out under memory pressure which helps to swap the deeper and wider neural networks with better accuracy but limited GPU memory. They model the deep learning computation as a dataflow graph, which performs joint optimization along 3 dimensions based on the given dataflow graph: operator scheduling, memory allocation, and swap decisions. They reduce the DNN’s memory consumption by 1) smartly swapping the model parameters that are updated at the end of an iteration and used by the next iteration, 2) carefully handling the intermediate results including activation, gradient, and error tensors, of which the latter two are only present in training but not in inference, and 3) managing the scratch space which is up to one gigabyte as a small fraction of total memory use.

% Grus \cite{wang-grus} analyzes the impact of several unified virtual memory (UVM) interfaces on graph workloads and proposes optimized adjustments for better performance. Shao et al.  \cite{scm-uvm} we attempt to analyze and explain the implications of GPU UVM oversubscription. They evaluate the performance sensitivity of applications with over-scribed memory size on GPU, and they find that co-running applications make memory competition worse in this case.  

% Soroush et al  \cite{co-optimizing} sets out to explore the hidden performance implication of GPU memory management methods of integrated CPU/GPU architecture. Through a series of experiments on micro-benchmarks and real-world workloads, they analyze application characteristics and develop a performance model that can predict system overhead for each memory management method.  They also propose a runtime scheduler that can significantly relieve the system memory pressure and reduce the multitasking co-run response time by conducting per-task memory management policy switching and kernel overlapping.

% Buddy Compression \cite{buddycompression}  makes novel use of compression to utilize a larger buddy memory from the host or disaggregated memory, effectively increasing the memory capacity of the GPU. 


% \subsubsection{GPU + SSD/NVMe}
% BAM
% GPU Direct-storage
% GPUDirect RMDA
% ZeRO-Infinity



% \subsubsection{Multi GPU}
% %COARSE
% %MC-DLA
% %Grinffin
% %LaySA


%LaySA Griffin MC-DLA COARSE Buddy ZeRO-Infinity GPUDirect Direct-storage BAM Soroush Grus Swap 


==> Contents/drop-6-Service-acceleration.tex <==
\section{Service-oriented Optimization }  \label{sec-service}





\subsection{Computation Modes}


%\textbf{A Comparison of Different Execution Models}

%Both single-node and distributed computing have been used for graph processing. As a complement to the two models, far memory provides a new option for scaling out memory with high performance. First, from the perspective of a single node, far memory provides a ready-to-use scheme for memory-intensive applications to oversubscribe memory, which outperforms disk-based I/O. Second, at the cluster level, far memory shows promise in further improving resource utilization especially for the SOTA shared-state schedulers like Omega\cite{omega}, Apollo\cite{apollo}, etc. To sum up, in the graph processing domain, far memory allows one to achieve better performance per bit in a complex execution environment.

%Tightly-coupled far memory can be viewed as a two-node 
%Wukong\cite{wukong} is a RDMA-friendly graph query model for low-latency graph processing on the InfiniBand network. 
%There are no works optimizing graph programs on the direct-connected far memory platforms due to the exorbitant hardware cost

Both single-node and distributed computing have been used for graph processing. As a complement to the two models, far memory provides a new option for scaling out memory with high performance.

\subsubsection{Far Memory vs. Single-Node Systems}

The traditional single-node graph processing system, with all data loaded in local memory, often shows the best performance\cite{ligra-2013,congra,graphit}. If the size of the graph is large, one can use disk storage as a memory extension\cite{gridgraph,chaos,mosaic}, as shown in Figure \ref{fig:background}-(b). However, this may come with considerable performance overhead even with a fast SSD. In contrast, far memory offers an attractive alternative to disk-based memory extension, especially in the cloud environment\cite{eurosys2020,asplos19software}. Far memory access shows lower performance degradation compared with disk I/O. On the other hand, faced with fluctuating workload demand, far memory represents a more convenient way to oversubscribe memory on demand. 

\subsubsection{Far Memory vs. Distributed Systems}
At the cluster level, far memory shows promise in further improving resource utilization especially for the SOTA shared-state schedulers like Omega\cite{omega}, Apollo\cite{apollo}, etc.

\subsection{Service-aware Far Memory Management}




\subsubsection{Elastic Computing on Far Memory}

Elastic applications typically have on-demand dynamic networking requirements. For instance, computing nodes in a disaggregated storage system access the data stored at the storage nodes across the network. System that requires elasticity means they need the ability to automatically scale according to application demands. 

KRCore \cite{wei2022krcore} is an RDMA library with a microsecond-scale control plane on commodity RDMA hardware for elastic computing. The key ideas include virtualizing pre-initialized kernel-space RDMA connections instead of creating one from scratch, and retrofitting advanced RDMA dynamic connected transport with static transport for both low connection overhead and high networking speed. 

Beldi \cite{zhang2020fault} proposes a library and runtime system for writing and composing fault-tolerant and transactional stateful serverless functions(SSFs). Beldi extends Olive, a recent frame-work that exposes an elegant abstraction to clients of cloud storage systems, and adapts its mechanisims to the stateful serverless functions in order to guarantee exactly-once semantics to workflows of SSFs. Beldi also adapts existing concurrency control and distributed commit protocols to support transactions over SSF workflows.



\subsection{Application-aware Far Memory Optimization}

There are plenty of works on running large-scale applications on memory-constrained systems. Some works \cite{shao-icpe, wang2018superneurons,zhang2018wonderland, gridgraph} analyze performance implications of classic memory-consuming workloads such as graph processing, AI model training, etc. Some works design specific memory access approaches based on read and write behavior and utilize data transfer channels to improve memory bandwidth utilization\cite{cao-drdram, wang-grus,fargraph}. Some works design memory-saving techniques and data offloading strategies on limited local memory and far memory space\cite{fargraph,wang-grus,wang-skywalker}. HyFarM\cite{hyfarm} can fit well with existing systems and support excavating the performance and efficiency potential of memory-constrained applications.


\subsubsection{Graph-aware Far Memory} 
Fargraph\cite{fargraph} analyzes the impact of graph processing workload on disaggregated architecture and proposes a graph-aware data segment offloading mechanism that can automally offload read-only edge-related data to RDMA-based far memory to reduce the overall data movement. In addition, They use optimal data segment splitting and asynchronous data buffering and prefetching to achieve graph iteration-friendly far memory access. 
FAMgraph\cite{fam-graph} uses a similar idea, which presents a semi-external graph processing system that leverages  the offloading of all the read-only edge data to efficiently tier data between local and remote memory.
Grus\cite{wang-grus} and Skywalker\cite{wang-skywalker} overscribe the GPU memory by utilizing CPU memory with unified virtual memory(UVM) on graph workloads and propose optimized adjustments for better performance. 

\subsubsection{DNN-supported Far Memory} 
To meet the strict service level agreement requirements of recommendation systems, the entire set of embeddings in recommendation systems needs to be loaded into the memory. However, as the model and dataset for production-scale recommendation systems scale up, the size of the embeddings is approaching the limit of memory capacity. Limited physical memory constrains the algorithms that can be trained and deployed, posing a severe challenge for deploying advanced inference systems.
Recent studies offload the embedding lookups into SSDs, which target the embedding-dominated recommendation models. RM-SSD\cite{recommendation-ssd} offloads the entire recommendation system into SSD with in-storage computing capability. The proposed SSD-side FPGA solution leverages a low-end FPGA to speed up both the embedding-dominated and MLP-dominated models with high resource efficiency. 

\subsubsection{Large Model Training}
 HET \cite{hetu-tencent} is a new system framework that significantly improves the scalability of huge embedding model training. They embrace skewed popularity distributions of embeddings and leverage an embedding cache to address the communication bottleneck. They also provides fine-grained consistency guarantees on a per-embedding basis. 
Angel-PTM \cite{Angel-PTM} is a productive deep learning system that can train extremely large-scale Transformer models with hierarchical memory efficiently. Angel-PTM  proposes fine-grained memory management via page abstraction between GPU, CPU and storage with a unified scheduling method that coordinates computations, data movements, and communications. Furthermore, Angel-PTM implements a lock-free updating mechanism to address the SSD I/O bottlenecks. 

% \textbf{DM Preference analysis. } The preference of external memory devices changed as new memory and storage devices develops. We also summarize the preference changes in each eras, as shown in Figure \ref{fig:bwandlatency}-(a). Intra-FMs such as HDD, SDD are preferred when the system requires much more memory space while Inter-FMs such as TCP/IP and RDMA NIC are preferred when the system requires lower latency and larger memory bandwidth. Nowadays, the preference for inter-node and intra-node connection tends to be smooth, as the performance of inter-node fabric-attached devices such as CXL, NVlink, RDMA,  and intra-node direct-connected devices such as NVM, disaggregated memory devices, and SSD become close to each other. In this case, the selection of far memory backend requires detailed consideration for higher overall efficiency.  
% Intra-FM can only  provide cluster-level elastic resource sharing through the network (i.e. Inter-FM) due to locality. 

==> Contents/table_copy.tex <==
% Kevin Lim et al. \cite{disaggregated-mem-isca09}
% LegoOS \cite{legoos}
% String Figure\cite{stringfigure}
% Clover\cite{pDPM-persistentmemory}
% Zombieland\cite{zombieland}
% ThymesisFlow\cite{thymesisflow}
% Clio\cite{clio}
% OCM\cite{optically-jpdc2022}
% BEACON\cite{beacon-micro22}
% MIND\cite{mind}
% Andres et al. \cite{asplos19software}
% TMO\cite{tmo}
% Infiniswap \cite{infiniswap}
% FastSwap\cite{icdcs19, FastSwap-github}
% Fastswap, CFM\cite{fastswap}
% Leap\cite{leap}
% Sherman\cite{wang2022sherman}
% Canvas \cite{canvas-nsdi23}
% Kona\cite{rethinking-asplos21}
% Panos et al.\cite{holistic2021ccgrid}
% HybridSwap\cite{hybridswap}
% XMemPod \cite{xmempod}
% MemLiner\cite{memliner}
% Semeru\cite{semeru}
% AIFM\cite{aifm}
% Jiffy\cite{jiffy-eurosys22}
% Pond\cite{pond-asplos23}\
% LITE \cite{lite}
% FaRM \cite{farm}
% Remote Region\cite{remoteRegion}
% FreeFlow\cite{freeflow}r
% AR-gRPC \cite{tensorflow-RDMA}  
% Mitosis\cite{mitosis-serverless}
% Medes \cite{saxena2022memory}
% Fargraph\cite{fargraph, fargraph+} 
% KRCore \cite{wei2022krcore}
% Beldi \cite{zhang2020fault}
% FAMgraph\cite{fam-graph}
% RM-SSD\cite{recommendation-ssd} 
% Swap Advisor\cite{swapadvisor}
% BAM \cite{bam} 
% ZeRO-Infinity \cite{Zero-infinity} 
% Buddy Compression\cite{buddycompression} 
% COARSE \cite{coarse-hpca22} 
%  MC-DLA \cite{micro2018beyond} 
%  Griffin \cite{griffin}
% LaySA\cite{zhao2021bridging} 
% Hybrid${^{2}}$\cite{hybrid2} 
% Memtrade\cite{memtrade}
% HyFarM\cite{hyfarm} 
% HET \cite{hetu-tencent}
% Angel-PTM \cite{Angel-PTM} 

% \checkmark 
% \scalebox{0.85}[1]{$-$}


\section{Classification of Related Works}
% 
% summarize for table.tex
\begin{itemize}
    \item 
\end{itemize}




\begin{table}[]\small
\caption{A summary of function on related works. $\checkmark$ means this aspect is carefully designed in the paper,  $\circ$ means this aspect is considered in the paper, $-$ is not considered. "NIC" means Network Interface Card. "CXL" is Computing express link. "TCO" means Total Cost of Ownership. "OCM" is Optically Connected Memory. "VM" represents Virtual Machine and "JVM" is Java Virtual Machine. "DL" is Deep Learning and "ML" is Machine Learning. "A/F" represents that the system considers anonymous pages and File-backed pages. "Fa" represents Failure and "Is" represents Isolation.  }
 \resizebox{\columnwidth}{!}{%
\begin{tabular}{!{\vrule width1.2pt}c!{\vrule width1.2pt}c|c|c|c|c|c|c|c!{\vrule width1.2pt}c|c|c|c|c!{\vrule width1.2pt}c|c|c|c|c|c!{\vrule width1.2pt}c|c|c|c!{\vrule width1.2pt}c|c|c|c!{\vrule width1.2pt}}%{|c|xxxxxxxx|xxxxx|xxxxxx|xxxx|}
 \hline

\multicolumn{1}{!{\vrule width1.2pt}c!{\vrule width1.2pt}}{} & \multicolumn{8}{c!{\vrule width1.2pt}}{\textbf{Far Memory Type (Local is DRAM)}} & \multicolumn{5}{c!{\vrule width1.2pt}}{\textbf{System Level}} & \multicolumn{6}{c!{\vrule width1.2pt}}{\textbf{Design Goals}} & \multicolumn{4}{c!{\vrule width1.2pt}}{\textbf{Granularity}} & \multicolumn{4}{c!{\vrule width1.2pt}}{\textbf{Programming}}\\ \hline
% Workload & \multicolumn{1}{c|}{\rotatebox{90}{PM(NVM)}} & \multicolumn{1}{c|}{\rotatebox{90}{CXL}} & \multicolumn{1}{c|}{\rotatebox{90}{RDMA}} & \multicolumn{1}{c|}{\rotatebox{90}{smartNIC (DPU,FPGA)}} & \multicolumn{1}{c|}{\rotatebox{90}{SSD}} & \multicolumn{1}{c|}{\rotatebox{90}{disk}} & \multicolumn{1}{c|}{\rotatebox{90}{GPU}} & \multicolumn{1}{c|}{\rotatebox{90}{Hybrid Memory}} & \multicolumn{1}{c|}{\rotatebox{90}{Hardware}} & \multicolumn{1}{c|}{\rotatebox{90}{Architecture} & \multicolumn{1}{c|}{\rotatebox{90}{OS}} & \multicolumn{1}{c|}{\rotatebox{90}{Runtime}} & \rotatebox{90}{Service} & \multicolumn{1}{c|}{\rotatebox{90}{Memory access latency}} & \multicolumn{1}{c|}{\rotatebox{90}{Data throughput}} & \multicolumn{1}{c|}{\rotatebox{90}{Security}} & \multicolumn{1}{c|}{\rotatebox{90}{Power  consumption}} & \multicolumn{1}{c|}{\rotatebox{90}{Application  performance }} & \multicolumn{1}{c|}{\rotatebox{90}{Resource  utilization}} \\ \hline
% \rule{0pt}{20pt} 
% \multicolumn{1}{|m{3cm}|}{Workload} 
\multicolumn{1}{!{\vrule width1.2pt}c!{\vrule width1.2pt}}{\begin{tabular}[c]{@{}c@{}}\textbf{Workload} \\  \\\end{tabular}} & \multicolumn{1}{c|}{\rotatebox{90}{PM (NVM)}} & \multicolumn{1}{c|}{\rotatebox{90}{CXL}} & \multicolumn{1}{c|}{\rotatebox{90}{Network Fabric (NIC)}} & \multicolumn{1}{c|}{\rotatebox{90}{Memory Controller}} & \multicolumn{1}{c|}{\rotatebox{90}{SSD}} & \multicolumn{1}{c|}{\rotatebox{90}{disk}} & \multicolumn{1}{c|}{\rotatebox{90}{GPU}} & \multicolumn{1}{c!{\vrule width1.2pt}}{\rotatebox{90}{Hybrid Memory}} & \multicolumn{1}{c|}{\rotatebox{90}{Hardware}} & \multicolumn{1}{c|}{\rotatebox{90}{Architecture}} & \multicolumn{1}{c|}{\rotatebox{90}{Operating System (OS)}} & \multicolumn{1}{c|}{\rotatebox{90}{Runtime  \& VM }} & \multicolumn{1}{c!{\vrule width1.2pt}}{\rotatebox{90}{Service}} & \multicolumn{1}{c|}{\rotatebox{90}{Ownership Cost (TCO)}} & \multicolumn{1}{c|}{\rotatebox{90}{Execution Latency}} & \multicolumn{1}{c|}{\rotatebox{90}{Data/task Throughput \quad}} & \multicolumn{1}{c|}{\rotatebox{90}{Power Consumption \quad}} & \multicolumn{1}{c|}{\rotatebox{90}{Isolation \& Failure  }} & \multicolumn{1}{c!{\vrule width1.2pt}}{\rotatebox{90}{Resource Utilization}} & \multicolumn{1}{c|}{\rotatebox{90}{Cache Line (64B)}} & \multicolumn{1}{c|}{\rotatebox{90}{Page Size (4K)}} & \multicolumn{1}{c|}{\rotatebox{90}{Large Page (2M)}}& \multicolumn{1}{c!{\vrule width1.2pt}}{\rotatebox{90}{Object (vary)}}  & \multicolumn{1}{c|}{\rotatebox{90}{Transparent}} & \multicolumn{1}{c|}{\rotatebox{90}{Cache Coherence}} & \multicolumn{1}{c|}{\rotatebox{90}{Costumed API usage}} & \multicolumn{1}{c!{\vrule width1.2pt}}{\rotatebox{90}{Parameter Conf.}}  \\ \hline
Memory Blade'09 \cite{disaggregated-mem-isca09} 
& $-$ & $-$  & $-$ & FGRA & $-$ & $-$ & $-$ &  $-$ 
& $\circ$  & $\checkmark$ & $-$ & $-$ &  $-$
&  $\checkmark$ &  $\checkmark$ & $-$  & $\checkmark$ & $-$ &  $-$ 
& $-$ & $\checkmark$ &$-$ & $-$  
&$\circ$  &$\checkmark$  & $-$  &$-$   \\ \hline

FaRM'14 \cite{farm}
& $-$ & $-$ & RDMA & $-$  & $\circ$ & $-$ & $-$ & $-$ 
& $-$ & $-$ & $-$ & $\checkmark$ & \begin{tabular}[c]{@{}c@{}} Read \\ Write\end{tabular}
& $-$ & $\checkmark$ & $\checkmark$ & $-$ & $-$ & $-$
& $-$ & $-$ & $-$ & $\checkmark$
&$-$  &$-$  &$\checkmark$  &$-$   \\ \hline

Holistic'15 \cite{holistic2021ccgrid}
& $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & NUMA
& $-$ & $-$ & $\checkmark$ & VM &   $-$
& $-$ & $-$ & $-$ & $-$ & $-$ & $\checkmark$
& $-$ & $\checkmark$ & $-$ &  $-$
& $\checkmark$   &$-$  &$-$  &$-$   \\ \hline

HybridSwap'15 \cite{hybridswap}
& $-$ & $-$ & $-$ & $-$  & $\checkmark$  & $-$ & $-$ & $-$
& $-$ & $-$ & $-$ & VM &  $-$
& $-$ & $\checkmark$ & $-$ & $-$ & $-$ & $-$ 
& $-$ & $\checkmark$  & $-$ & $-$
&$\checkmark$ &$-$  &$-$  &$-$   \\ \hline
% XMemPod \cite{xmempod}& $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ &  & $-$ & $-$ & $-$ & $-$ &  & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ &  &$-$  &$-$  &$-$  &$-$   \\ \hline

LITE'17 \cite{lite}
& $-$ & $-$ & RDMA & $-$  & $-$  & $-$ & $-$ & $-$ 
& $-$ & $-$ & $\checkmark$ & $\checkmark$ & \begin{tabular}[c]{@{}c@{}} Read \\ Write\end{tabular}
& $-$ & $\checkmark$ & $\checkmark$ & $-$ & $-$ & $\checkmark$
& $-$ & $-$ & $-$ & $\checkmark$
&$-$  &$-$  &$\checkmark$  &$-$   \\ \hline

Infiniswap'17 \cite{infiniswap}
& $-$ & $-$ & RDMA & $\checkmark$ & $-$ & $-$ & $-$ & $-$
& $-$ & $-$ & $\checkmark$ & $-$ & $-$ 
& $-$ & $\checkmark$ & $-$ & $-$ & Fa &  $-$
& $-$ & $\checkmark$ &$-$ & $-$ 
&$\checkmark$  &$-$  &$-$  &$-$   \\ \hline

LegoOS'18 \cite{legoos} 
& $\checkmark$ & $-$   & $-$   & $-$ & $\circ$ & $\circ$ & $\circ$  & $-$  
& $-$ & $\circ$  & $\checkmark$ & $\circ$  & $-$ 
& $\checkmark$ & $\checkmark$ & $-$ & $-$ & Fa &  $-$ 
& $-$ & $\checkmark$  &$-$ & $-$  
&$\checkmark$  &$-$  &$-$  & $-$   \\ \hline

Zombieland'18 \cite{zombieland}
& $-$ & $-$ & RDMA & ACPI & $-$ & $-$ & $-$ & $-$ 
& $-$ & $-$ & $\circ$ & $\checkmark$ & $-$
& $-$  & $\checkmark$  & $-$ & $\checkmark$  & $-$ &  $-$ 
& $-$ & $\checkmark$ &$-$ & $-$  
&$\checkmark$ &$-$  &$-$  &$-$   \\ \hline

Remote Region'18 \cite{remoteRegion}
& $-$ & $-$ & RDMA & $-$  & $\circ$ & $-$ & $-$ & $-$ 
& $-$ & $-$ & $-$ & $\checkmark$ & $-$
& $-$ & $\checkmark$ & $\checkmark$ & $-$ & Is & $-$
& $-$ & $\checkmark$ & $-$ & $\checkmark$
&$-$  &$-$  &$\checkmark$  &$\checkmark$    \\ \hline


AR-gRPC'18 \cite{tensorflow-RDMA}  
& $-$ & $-$ & RDMA & $-$  & $-$ & $-$ & $-$ & $-$ 
& $-$ & $-$ & $-$ & $\checkmark$ & Tensorflow
& $-$ & $\checkmark$ & $\checkmark$ & $-$ & Is & $-$
& $-$ & $-$ & $-$ & $\checkmark$
&$-$  &$-$  &$\checkmark$  &$\checkmark$    \\ \hline

 MC-DLA'18 \cite{micro2018beyond} 
 & $-$ & $-$ & \begin{tabular}[c]{@{}c@{}} PCIe\\ Switch\end{tabular} & $-$ & $-$ & $-$ & $\checkmark$  & $-$
 & $-$ & $\checkmark$  & $-$ & $-$ & \begin{tabular}[c]{@{}c@{}} DL \\ Training\end{tabular}
 & $-$ & $\checkmark$ & $\checkmark$ & $\checkmark$  & $-$ & $-$ 
 & $-$ & $\checkmark$  & $-$ & $-$
 &$-$  &$-$  &$\checkmark$  &$-$   \\ \hline
 
String Figure'19 \cite{stringfigure} 
& $-$ & $-$ & $-$ & RTL & $-$ & $-$ & $-$ & HMC  
& $\checkmark$ & $\checkmark$ & $-$ & $-$ &   
& $-$ & $-$ & $\checkmark$ & $\checkmark$ & $-$ & $-$ 
&$\checkmark$  & $-$ & $-$ &$-$  
&$-$  &$\checkmark$ &$-$  &$-$   \\ \hline

Zswap'19 \cite{asplos19software,zswapkernel}
& $-$ & $-$ & $-$ & $-$ & $-$ & $\checkmark$  & $-$ & $-$
& $-$ & $-$ & $\checkmark$ & $-$ & $-$
& $\checkmark$  & $\checkmark$  & $-$ & $-$ & $-$ &  $-$
& $-$ & $\checkmark$ &$-$ & $-$ 
&$\checkmark$  &$-$  &$-$  &$-$   \\ \hline

FreeFlow'19 \cite{freeflow}
& $-$ & $-$ & vRDMA & $-$  & $-$ & $-$ & $-$ & $-$ 
& $-$ & $-$ & $-$ & $\checkmark$ & Container
& $-$ & $\checkmark$ & $\checkmark$ & $-$ & Is & $-$
& $-$ & $-$ & $-$ & $\checkmark$
&$-$  &$-$  &$\checkmark$  &$\checkmark$    \\ \hline

Leap'19 \cite{leap} 
& $-$ & $-$ & RDMA & $\checkmark$ & $\checkmark$ & $-$ & $-$ & $-$ 
& $-$ & $-$ & $-$ & $\checkmark$ & $-$
& $-$ & $\checkmark$ & $\checkmark$ & $-$ & $-$ & $-$
& $-$ & $\checkmark$ & $-$ & $-$
&$-$  &$-$  &$\checkmark$  &$-$   \\ \hline


Clover'20 \cite{pDPM-persistentmemory} 
& $\checkmark$ & $-$ & RDMA & $-$ & $-$ & $-$ & $-$ & $-$
& $-$ & $-$ & $-$ & $\checkmark$ & \begin{tabular}[c]{@{}c@{}}Kv Store\end{tabular}
& $-$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $-$ &  $-$
& $-$ & $-$ &$-$ & $\checkmark$ 
&$-$  &$-$  & $\checkmark$ &$-$   \\ \hline


ThymesisFlow'20 \cite{thymesisflow}
& $-$ & $\circ$  & OpenCAPI & FPGA & $-$ & $-$ & $\circ$  &$-$ 
& $\checkmark$ & $\circ$  & $\checkmark$ & $-$ & $-$ 
& $-$ & $-$ & $\checkmark$ & $-$ & $-$ & $\checkmark$
& $\circ$  &$\checkmark$ &$-$ & $-$  
&$\checkmark$  &$\circ$  &$-$  &$-$   \\ \hline


Fastswap, CFM'20 \cite{fastswap}
& $-$ & $-$ & RDMA & $\checkmark$ & $\checkmark$ & $-$ & $-$ & $-$
& $-$ & $-$ & $\checkmark$ & $\checkmark$ & $-$ 
& $\checkmark$ & $\checkmark$ & $\checkmark$ &$-$ & $-$ &  $-$
& $-$ & $\checkmark$ &$-$ & $-$ 
&$\checkmark$  &$-$  &$-$  &$\checkmark$   \\ \hline


Semeru'20 \cite{semeru}
& $-$ & $-$ & RDMA & $\checkmark$ & $\circ$  & $-$ & $-$ &$-$
& $-$ & $-$ & $-$ & JVM & $-$
& $-$ & $\checkmark$  & $\checkmark$  & $-$ & $-$ & $\checkmark$ 
& $-$ & $\checkmark$  & $-$ &  $\checkmark$ 
&$-$  &$-$  &$\checkmark$   &$-$   \\ \hline

AIFM'20 \cite{aifm}
& $-$ & $-$ & RDMA & $-$ & $-$ & $-$ & $-$ &  $-$
& $-$ & $-$ & $-$ & $\checkmark$ & $-$ 
& $-$ & $\checkmark$ & $\checkmark$ & $-$ & $-$ & $-$ 
& $-$ & $-$ & $-$ & $\checkmark$
&$-$  &$-$  &$\checkmark$  &$-$   \\ \hline


Swap Advisor'20\cite{swapadvisor}
& $-$ & $-$ & NVLink & $-$ & $\checkmark$  & $-$ & $\checkmark$ & $-$
& $-$ & $-$ & $-$ & $\checkmark$ &\begin{tabular}[c]{@{}c@{}} DL \end{tabular}
& $-$ & $\checkmark$  & $\checkmark$  & $-$ & $-$ & $-$ 
& $-$ & $\checkmark$ & $-$ & $-$ 
&$\checkmark$ &$-$  &$-$  &$\checkmark$  \\ \hline

 Buddy Compression'20 \cite{buddycompression} 
& $-$ & $-$ & NVLink & $-$  & $\checkmark$ & $-$ & $\checkmark$  & $-$
& $-$ & $-$ & $-$ &$\checkmark$  & $-$
& $-$ & $\checkmark$ & $\checkmark$  & $-$ & $-$ & $-$
& $-$ & $\checkmark$ & $-$ & $-$
&$-$  &$\checkmark$  &$-$  &$-$   \\ \hline

 Griffin'20 \cite{griffin}
 & $-$ & $-$ & PCIe & IOMMU & $-$ & $-$ & $\checkmark$ & NUMA
 & $\checkmark$  & $\checkmark$  & $-$ & $-$ & $-$ 
 & $-$ & $\checkmark$  & $-$ & $-$ & $-$ & $-$ 
 & $-$ & $\checkmark$  & $-$ & $-$ 
 &$\checkmark$   &$-$  &$-$  &$-$   \\ \hline

Hybrid${^{2}}$'20 \cite{hybrid2} 
& $-$ & $-$ & DIMM & $-$ & $-$ & $-$ & $-$ & \begin{tabular}[c]{@{}c@{}} 3D-stacked \\ DRAM\end{tabular}
& $\checkmark$ & $\checkmark$ & $-$ & $-$ & $-$
& $\checkmark$ & $\checkmark$ & $\checkmark$ & $-$ & $-$ & $-$ 
& $-$ & $\checkmark$ & $-$ & $\checkmark$ 
&$-$  &$-$  &$\checkmark$  & $\checkmark$  \\ \hline


MIND'21 \cite{mind}
& $-$ & $-$ & Switch & ASIC & $-$ & $-$ & $-$ & $-$
&$\circ$  &$\checkmark$ & $-$ & $-$ & $-$
& $-$ & $\checkmark$ & $-$ & $-$ & Fa &  $-$
& $-$ & $\checkmark$ &$-$ & $-$ 
&$\checkmark$  &$-$  &$-$  &$-$   \\ \hline

XMemPod'21 \cite{icdcs19, FastSwap-github,xmempod}
& $-$ & $-$ & RDMA & $\checkmark$ & $\checkmark$ & $-$ & $-$ & $-$
& $-$ & $-$ & $\checkmark$ & VM & $-$ 
& $-$ & $\checkmark$ & $-$ & $-$ & Is &  $-$
& $-$ & $\checkmark$ &$-$ & $-$ 
&$\checkmark$  &$-$  &$-$  &$-$   \\ \hline

Kona'21 \cite{rethinking-asplos21}
& $-$ & $\checkmark$ & RDMA & FPGA & $-$ & $-$ & $-$ & $-$  
& $-$ & $\checkmark$ & $-$ & $\checkmark$ & $-$  
& $-$ & $\checkmark$ & $-$ & $-$ & Fa & $-$
& $\checkmark$  & $-$ & $-$ & $-$    
&$\checkmark$  &$\checkmark$  & $\checkmark$  &$-$   \\ \hline

ZeRO-Infinity'21 \cite{Zero-infinity} 
& $-$ & $-$ & NVLink &  $-$ & $\checkmark$ & $-$ & $\checkmark$  & $-$
& $-$ & $-$ & $-$ &$\checkmark$  & \begin{tabular}[c]{@{}c@{}} DL \end{tabular}
& $-$ & $\checkmark$ & $\checkmark$  & $-$ & $-$ & $-$
& $-$ & $\checkmark$ & $-$ & $-$
&$-$  &$\checkmark$  &$-$  &$-$   \\ \hline
 
LaySA'21 \cite{zhao2021bridging} 
& $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $\checkmark$ & $-$
& $-$ & $-$ & $-$ & $-$ & \begin{tabular}[c]{@{}c@{}} DL \\ Training\end{tabular}
& $-$ & $\checkmark$  & $\checkmark$  & $-$ & $-$ & $-$ 
& $-$ & $\checkmark$  & $-$ & $-$
&$\checkmark$   &$-$  &$-$  &$-$   \\ \hline

HET'21 \cite{hetu-tencent} 
& $-$ & $-$ & $-$ & $-$  & $-$ & $\checkmark$ & $\checkmark$  & $-$
& $-$ & $-$ & $-$ &$\checkmark$  & \begin{tabular}[c]{@{}c@{}} ML \\ Training\end{tabular}
& $\checkmark$ & $\checkmark$ & $-$  & $-$ & $-$ & $-$
& $-$ & $\checkmark$ & $-$ & $-$
&$-$  &$\checkmark$  &$-$  &$-$   \\ \hline


Memtrade'21 \cite{memtrade}
& $-$ & $-$ & $-$ & $-$ & $\checkmark$ & $\checkmark$ & $-$ & $-$
& $-$ & $-$ & $-$ & VM & $-$
& $\checkmark$ & $\checkmark$ & $-$ & $-$ & $-$ & $\checkmark$
& $-$ & $\checkmark$ & $-$ & $-$
&$-$  &$-$  &$\checkmark$ &$-$   \\ \hline


TMO'22 \cite{tmo}
& $-$ & $-$ & $-$ & $-$ & $\checkmark$ & $\checkmark$ & $-$ & $-$
& $-$ & $-$ & $\checkmark$ & $-$ & $-$
& $\checkmark$ & $\checkmark$ & $\checkmark$ & $-$ & $-$ & $-$
& $-$ & A/F & $-$ & $-$
&$\checkmark$  &$-$  &$-$  &$\checkmark$  \\ \hline

Sherman'22 \cite{wang2022sherman}
& $\circ$ & $-$ & RDMA & $-$ & $-$ & $-$ & $-$ & $-$ 
& $-$ & $-$ & $-$ & $\checkmark$ & \begin{tabular}[c]{@{}c@{}}Read/ \\ Write\end{tabular}
& $-$ & $\checkmark$ & $\checkmark$ & $-$ & $-$ &  $-$ 
& $-$ & $-$ &$-$ & $\checkmark$  
&$-$  &$-$  &$\checkmark$  &$-$   \\ \hline

Teleport'22\cite{teleport-sigmod}
& $-$ & $-$   & RDMA    & $-$ & $\circ$ & $\circ$ & $\circ$  & $-$  
& $-$ & $\circ$  & $\checkmark$ & $\circ$  & $-$ 
& $\checkmark$ & $\checkmark$ & $-$ & $-$ & $-$  &  $-$ 
& $-$ & $\checkmark$  &$-$ & $-$  
&$-$  &$\checkmark$  &$\checkmark$  & $-$   \\ \hline

Jiffy'22 \cite{jiffy-eurosys22}
& $-$ & $-$ & RDMA &$\checkmark$ &$\checkmark$& $-$ & $-$ & $-$
& $-$ & $-$ & $-$ & $\checkmark$ & Serverless
& $\checkmark$ & $\checkmark$ & $-$ & $-$ & $-$ & $\checkmark$ 
& $-$ & $-$ & $-$ & $\checkmark$
&$-$  &$-$  &$\checkmark$   &$\checkmark$   \\ \hline

Clio'22 \cite{clio}
& $-$ & $-$ & RDMA & FPGA  & $-$ & $-$ & $-$ & $-$ 
& $\circ$ & $\checkmark$ & $-$ & $-$ & $-$  
& $-$ & $\checkmark$ & $\checkmark$ & $\checkmark$ & $-$ & $-$
& $-$ & $\circ$ & $-$ & $\checkmark$
&$-$  &$-$  &$\checkmark$ &$-$   \\ \hline

OCM'22 \cite{optically-jpdc2022}
& $-$ & $-$  & Optical & $-$ & $-$ & $-$ & $-$ & OCM
& $\checkmark$ & $\checkmark$ & $-$ & $-$ & $-$
& $-$ & $\checkmark$& $\checkmark$ & $\checkmark$ & $-$ &  $-$ 
& $\checkmark$ & $-$ &$-$ & $-$  
&$\checkmark$ &$-$  &$-$  &$-$   \\ \hline

BEACON'22 \cite{beacon-micro22}
& $-$ & $\checkmark$ & $-$ & $-$ & $-$ & $-$ & $-$ & $\circ$ 
& $\circ$ & $\checkmark$ & $-$ & $-$ & \begin{tabular}[c]{@{}c@{}}Genome \\ Analysis\end{tabular}
& $-$ & $\checkmark$ & $-$ & $\circ$ & $-$ &  $-$ 
& $\checkmark$ & $-$ &$-$ & $-$  
& $-$  &$-$  &$\checkmark$  & $\checkmark$  \\ \hline

MemLiner'22 \cite{memliner}
& $-$ & $-$ & RDMA & $\checkmark$  & $-$ & $-$ & $-$ & $-$  
& $-$ & $-$ & $-$ & JVM & $-$ 
& $\checkmark$  & $\checkmark$  & $-$ & $-$ & $-$ & $-$ 
& $-$ & $-$ & $-$ &  $\checkmark$  
&$-$  &$\circ$  & $\checkmark$   &$-$   \\ \hline

Mitosis'22\cite{mitosis-serverless}
& $-$ & $-$ & RDMA & $-$  & $-$ & $-$ & $-$ & $-$ 
& $-$ & $-$ & $\checkmark$ & $-$ & Serverless
& $-$ & $\checkmark$ & $\checkmark$ & $-$ &Is & $-$
& $-$ & $-$ & $-$ & $\checkmark$
&$-$  &$-$  &$\checkmark$  &$\checkmark$    \\ \hline

Medes'22 \cite{saxena2022memory}
& $-$ & $-$ & RDMA & $-$  & $-$ & $-$ & $-$ & $-$ 
& $-$ & $-$ & $-$ & $\checkmark$ & Serverless
& $\checkmark$ & $\checkmark$ & $\checkmark$ & $-$ &Is & $-$
& $-$ & $\checkmark$ & $-$ & $\circ$
&$-$  &$-$  &$\checkmark$  &$\checkmark$    \\ \hline

Fargraph'22 \cite{fargraph, fargraphplus} 
& $-$ & $-$ & RDMA & $\checkmark$  & $\checkmark$ & $-$ & $-$ & 
& $-$ & $-$ & $-$ & $\checkmark$ & Graph
& $\checkmark$ & $\checkmark$ & $\checkmark$ & $-$ & $-$ & $-$
& $-$ & $-$ & $-$ & $\checkmark$ 
&$-$  &$-$  & $\checkmark$  &$-$   \\ \hline


FAMgraph'22\cite{fam-graph}
& $-$ & $-$ & RDMA & $\checkmark$  & $\checkmark$ & $-$ & $-$ & 
& $-$ & $-$ & $-$ & $\checkmark$ & Graph
& $\checkmark$ & $\checkmark$ & $\checkmark$ & $-$ & $-$ & $-$
& $-$ & $-$ & $-$ & $\checkmark$ 
&$-$  &$-$  & $\checkmark$  &$-$   \\ \hline

KRCore'22 \cite{wei2022krcore}
& $-$ & $-$ & RDMA & $-$ & $-$ & $-$ & $-$ & $-$
& $-$ & $-$ & $\checkmark$& $-$ & Elastic
& $-$ & $\checkmark$  & $\checkmark$ & $-$ & $-$ & $-$ 
& $-$ & $-$ & $-$ & $\checkmark$
&$-$  &$-$  &$\checkmark$  &$-$   \\ \hline

RM-SSD'22\cite{recommendation-ssd} 
& $-$ & $-$ & FPGA & $\checkmark$  & $-$ & $-$ & $-$ &$-$   
& $\checkmark$ & $\circ$ & $-$ & $-$ & $-$
& $-$ & $\checkmark$ & $\checkmark$ & $-$ & $-$ & $-$ 
& $-$ & $\checkmark$  & $-$ & $-$
&$-$  &$-$  & $\checkmark$  &$-$   \\ \hline

COARSE'22 \cite{coarse-hpca22} 
& $-$ & $-$ & CCI & FPGA & $-$ & $-$ & $\checkmark$  & $-$
& $-$ & $-$ & $-$ & $-$ & \begin{tabular}[c]{@{}c@{}} DL \\ Training\end{tabular}
& $-$ & $\checkmark$ & $\checkmark$  & $-$ & $-$ & $-$
& $-$ & $\checkmark$ & $-$ & $-$
&$-$  &$\checkmark$  &$-$  &$-$   \\ \hline

HyFarM'22 \cite{hyfarm}
& $-$ & $-$ & RDMA & $-$ & $\checkmark$ & $\checkmark$ & $-$ & $-$
& $-$ & $-$ & $-$ & $\checkmark$  & $-$
& $\checkmark$  & $\checkmark$  & $-$ & $-$ & $-$ & $\checkmark$ 
& $-$ & A/F & $-$ & $-$
& $\checkmark$ &$-$  &$-$  &$\checkmark$   \\ \hline

Canvas'23 \cite{canvas-nsdi23}
& $-$ & $-$ & RDMA & $-$ & $-$ & $-$ & $-$ & $-$
& $-$ & $-$ & $\checkmark$  & $\checkmark$  & $-$
& $-$ & $\checkmark$ & $-$ & $-$ & Is & $-$
& $-$ & A/F  & $-$ &  $-$
&$\checkmark$  &$-$  &$-$  &$\checkmark$    \\ \hline


BAM'23 \cite{bam}
& $-$ & $-$ & $-$ &  $-$ & $\checkmark$ & $-$ & $\checkmark$  & $-$
& $-$ & $-$ & $-$ &$\checkmark$  & $-$
& $-$ & $\checkmark$ & $\checkmark$  & $-$ & $-$ & $-$
& $-$ & $\checkmark$ & $-$ & $-$
&$-$  &$\checkmark$  &$-$  &$-$   \\ \hline

GIDS'23 \cite{GIDS}
& $-$ & $-$ & $-$ &  $-$ & $\checkmark$ & $-$ & $\checkmark$  & $-$
& $-$ & $-$ & $-$ &$\checkmark$  & $-$
& $-$ & $\checkmark$ & $\checkmark$  & $-$ & $-$ & $-$
& $-$ & $\checkmark$ & $-$ & $-$
&$-$  &$\checkmark$  &$-$  &$-$   \\ \hline

Helios'23 \cite{helios} 
& $-$ & $-$ & $-$ &  $-$ & $\checkmark$ & $-$ & $\checkmark$  & $-$
& $-$ & $-$ & $-$ &$\checkmark$  & $-$
& $-$ & $\checkmark$ & $\checkmark$  & $-$ & $-$ & $-$
& $-$ & $\checkmark$ & $-$ & $-$
&$-$  &$\checkmark$  &$-$  &$-$   \\ \hline

Angel-PTM \cite{Angel-PTM} 
& $-$ & $-$ & $-$ & $-$  & $\checkmark$ & $-$ & $\checkmark$  & HBM
& $-$ & $-$ & $-$ &$\checkmark$  & \begin{tabular}[c]{@{}c@{}} LLM \\ Training\end{tabular}
& $\checkmark$  & $\checkmark$ & $\checkmark$  & $-$ & $-$ & $-$
& $-$ & $\checkmark$ & 4MB & $-$
&$-$  &$\checkmark$  &$-$  &$-$   \\ \hline

Pond'23 \cite{pond-asplos23}
& $-$ & $\checkmark$ & \begin{tabular}[c]{@{}c@{}} CXL \\ Switch\end{tabular} & $-$ & $-$ & $-$ & $-$  & NUMA
& $\checkmark$  & $-$ & $-$ & VM  & $-$
& $\checkmark$& $\checkmark$& $-$ & $-$ & $-$ &  $\checkmark$ 
& $-$ &$\checkmark$ &  $-$ &  $-$
& $\checkmark$  & $\circ$  &$-$  &$-$   \\ \hline

\end{tabular}%
}
\end{table}


% Beldi \cite{zhang2020fault} 
% & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ &  
% & $-$ & $-$ & $-$ & $-$ & 
% & $-$ & $-$ & $-$ & $-$ & $-$ & $-$ 
% & $-$ & $-$ & $-$ & 
% &$-$  &$-$  &$-$  &$-$   \\ \hline


